Large Language Models as Minecraft Agents

In this work we examine the use of Large Language Models (LLMs) in the challenging setting of acting as a Minecraft agent. We apply and evaluate LLMs in the builder and architect settings, introduce clarification questions and examining the challenges and opportunities for improvement. In addition, we present a platform for online interaction with the agents and an evaluation against previous works.

==> methods_v1.tex <==
\section{Methodology}

The approach used in this work is inspired by the ``Collaborative Builder Task'' \cite{narayan2019collaborative} in which two agents collaborate in a voxel based world to build a structure.  The \textit{architect} is given a target world structure, and provides natural language instructions to a \textit{builder}, who cannot see the target structure, to place blocks to achieve that goal structure. Unlike the majority of previous approaches, both agents are able to provide and answer questions.

The builder agent operates as follows:
item The initial prompt contains instructions for the task, constraints of the world ($min/max$ for $x,y,z$), coordinate mappings (east/south/west/north) and requests that the LLM respond in a specified JSON format only (see \ref{sec:builderprompt} for full prompt).  Following the initial prompt, on each turn, the agent consumes an utterance (instruction) and produces a sequence of actions in addition to an optional clarification question in the originally specified format.  This JSON encoded representation is used to directly update the world. If the result does not constitute a valid JSON response it is disregarded.
The builder is evaluated against IGLU RL baseline sub-task. We evaluate the agent based on its ability to interpret a natural language instruction and produce the correct 3D coordinates and colours for the target structure (not manoeuvre an agent in a 3D space to interact with the world and realise that target structure).


The closest work to our methodology is \cite{mehta2023improving}, similarly we focus solely on the language component of this task. We do not examine the task of manipulating an agent to place blocks as done in previous tasks \cite{narayan2019collaborative,jayannavar2020learning,shi2022learning}, as it is the language element that we are most interested in.

The architect differs slightly from the builder.
The prompt, along with architect specific instructions, contains the target state of the world (see \ref{sec:architectprompt}). Following the initial prompt the architect consumes every utterance given by the builder, along with the current state of the world encoded in a structured JSON format.  The target structures are taken from the ``Collaborative Builder Task'' dataset \cite{narayan2019collaborative} and evaluated empirically through repeated interactions. 


%\begin{itemize}
%\item description
%\item prompts
%\item interactive website
%\end{itemize}

==> notes.tex <==
% THIS IS MOSTLY ALL WRONG
%\todo{next bit is wrong}
%In the prior work, the challenges identified are almost entirely related to the language understanding component \cite{narayan2019collaborative}. From a builder perspective, the prior work points to the use of reference, ellipsis and clarification questions. We focus solely on that area of research in this work.

%The reinforcement learning challenge is largely solved for this type of task.  Beyond navigating an agent in a constrained world to build a target structure, current Minecraft agents can navigate entire worlds and build cities CITATIONS.

%In the IGLU baseline, these are addressed separately, which inspired our evaluation method 

%block world experiment \cite{bisk2018learning}

%\textbf{Grounding} is the application of a model to link an environment outside the original training goals. Here, we attempt to ground dialog to a voxel based Minecraft like world, interacting with the model using $x,y,z$ coordinates and colours. It is very unlikely this task featured anywhere in the original LLMs training goals. We can also produce new structures and dialog CITATIONS.


%\textbf{Abstract symbolism and structure} comes naturally to humans. 
%In the Minecraft dialog task, frequent use of symbolism is applied. For example, a participant might use phrases such as ``L-shaped'' (as mentioned in \cite{narayan2019collaborative}), which although could easily be described through symbolism, or a rule based system, can't necessarily be inferred through the semantic knowledge of an LLM.

\todo{THIS ISN'T THE CURRENT THINKING, ALL WRONG: }
\textbf{Planning}...
\begin{itemize}
\item accomplishing the task of building a complex structure is best divided into a series of small structures
\item determining the optimum method to communicate or approach the task in itself is non-trivial
\item \textit{Voyager} uses LLMs to acquire new skills, crafting and world navigation \cite{wang2023voyager}.  They do not target the creation of specific structures.
\item other planning work in LLMs
\end{itemize}

\begin{itemize}
\item LLMs in other roles (particularly grounding LLMs)
\item reinforcement learning and why this isn't looked at here
\item Ask and answer clarification questions in dialogue
\item interpretation of nlp instructions
\item prior work (e.g. bap model)
\item architect and builder
\end{itemize}

There is much work in reinforcement learning Work using minecraft agents.


%The IGLU competition had a classification task for clarification
%questions, and a work following on from the original builder agent work \cite{narayan2019collaborative},
%a separate work added further modifications to include label denoting when an utterance required clarification \cite{shi2022learning}.
%There is prior work looking at generating natural language questions using a fine tuned BART model \cite{mehta2023improving}.
